Pano: Optimizing 360{\deg} Video Streaming with a Better Understanding of Quality Perception

Streaming 360{\deg} videos requires more bandwidth than non-360{\deg} videos. This is because current solutions assume that users perceive the quality of 360{\deg} videos in the same way they perceive the quality of non-360{\deg} videos. This means the bandwidth demand must be proportional to the size of the user's field of view. However, we found several qualitydetermining factors unique to 360{\deg}videos, which can help reduce the bandwidth demand. They include the moving speed of a user's viewpoint (center of the user's field of view), the recent change of video luminance, and the difference in depth-of-fields of visual objects around the viewpoint. This paper presents Pano, a 360{\deg} video streaming system that leverages the 360{\deg} video-specific factors. We make three contributions. (1) We build a new quality model for 360{\deg} videos that captures the impact of the 360{\deg} video-specific factors. (2) Pano proposes a variable-sized tiling scheme in order to strike a balance between the perceived quality and video encoding efficiency. (3) Pano proposes a new qualityadaptation logic that maximizes 360{\deg} video user-perceived quality and is readily deployable. Our evaluation (based on user study and trace analysis) shows that compared with state-of-the-art techniques, Pano can save 41-46% bandwidth without any drop in the perceived quality, or it can raise the perceived quality (user rating) by 25%-142% without using more bandwidth.

==> intro_dep.tex <==
%!TEX root = main.tex

\section{Introduction}


%A desirable video streaming protocol should maximize user-perceived video quality under dynamic network conditions.
%A key concern in video streaming is how to optimize video quality under fluctuating network bandwidth.
%On one hand, if the bandwidth is stable, one can maximize the quality (\eg high resolution, no rebuffering) by aggressively eliminating the pixel-level spatio-temporal redundancies.
%On the other hand, encoding the video too aggressively would make it hard to switch the quality level quickly enough to fully utilize the fluctuating bandwidth.
%A case-in-point of this tradeoff is DASH~\cite{??,??,??}, which recently took hold as the mainstream video protocol. 
%It balances the encoding efficiency and adaptation by splitting the video to fixed-length chunks (4-10 seconds) each encoded in discrete quality levels, allowing it to switch quality at chunk boundaries.

%The recent surge of \vr videos poses new challenges.
\vr videos are coming to age; most major content providers have rolled out \vrvideo-based applications~\cite{facebook,Google,Hulu,Vimeo,Netflix,Youku,iQiyi}.
At the same time, streaming \vr videos is arguably more challenging than streaming non-\vr videos.
To create an immersive experience, \vr videos must cover a larger area in high resolution than traditional videos without any stall~\cite{att,Gaddam}.
%\guanyu{
\edited{To put it into perspective, let us consider a standard HD video\jc{can we put the video online and give a url pointer?} (40 pixels-per-degree, PPD) displayed on a desktop screen (an area of $\sim$48\textdegree-by-27\textdegree in the \vr view), and streaming it takes about 2Mbps. 
In contrast, If we stream a \vr video (an entire panoramic view) with the same PPD and same content within the 48\textdegree-by-27\textdegree area, it will take 80Mbps, a 40-fold increase in bandwidth consumption.
% Even with a state-of-the-art \vrvideo solution~\cite{Flare} which only sends the predicted viewport, offering the same PPD still takes over 14.8Mbps, a 7.5-fold inflation (let alone buffering due to viewport prediction error). 
}




\xinggong{One question is risen: is it possible to deliver panoramic video to user with the same quality and bit-rate as non-VR HD video? Although many viewport-driven approaches have been proposed, but they are fall short of this aim. For a viewport with $100$\textdegree-by-$90$\textdegree, it needs $4,000$ pixels to offer same PPD as HD. It means at least 4K or more ultra-high-definition video is required to obtain the same viewport quality as traditional non-VR HD video. But 4K video consumes about two times bitrates of the traditional HD video. It is impossible for viewport-driven approach to achieve the aim. The bit-rate of viewport-driven should be half-cut at least. 
}
%\guanyu{since viewport in \vrvideo display is usually $\sim$98\textdegree-by-100\textdegree, 7.5$\times$ larger than that in traditional video display}.
%streaming a one-minute \vr video~\cite{give the url} as a regular HD video takes only 18 MB, whereas streaming it as a \vr video using state-of-the-art \vr streaming protocol~\cite{Flare} takes \fillme MB, a \fillme$\times$ increase in bandwidth consumption.
%Although one can save bandwidth by streaming only the area facing the viewer, doing so would (1) require accurately tracking the viewpoint movements which itself is not trivial, and (2) force the encoder to use shorter video chunks (\eg one second) to keep up with the movements of the viewpoint, which significantly reduces the coding efficiency and thus increases the bandwidth consumption.

% A key limiting factor in existing \vr video streaming solutions is that 
% %they have largely relied on the same QoE (quality of experience) model from non-\vr videos. 
% they assume users perceive the quality of \vr videos in the same way as they perceive traditional video quality (\ie without interactive behaviors, such as {\color{red} head movement}).
%, which fundamentally limits the room for improvement of \vr videos.
% \xinggong{clarifying the model of non-VR video: pixel-level distortion without considering human interactive behaviors }
%At a high level, the QoE model describes the correlation between how a video is presented to the viewer (\eg pixel-level differences to the original feed) and the user-perceived satisfaction, or QoE.
Many prior papers (\eg~\cite{Flare, ClusTile, viewpoint-driven1, viewpoint-driven5, Fan2017Fixation, Corbillon2017Viewport, Sreedhar2017Viewport}) have explored a viewport-driven approach: streaming only the region facing the viewer, \ie the viewport, or giving higher quality level to the viewport region.
%A notable exception is that the perceived QoE of a spatial area also depends on the region's distance to user's real-time viewpoint (\eg~\cite{distance}), so one can save bandwidth by streaming only the area facing the viewer.
Despite its sizable improvements over streaming a \vr video in its entirety, this approach alone is not sufficient to stream the video as efficiently as traditional non-\vr videos.
First, any prediction error of viewpoint movements can cause the re-buffering or quality drops;
Second, to stream the dynamic viewport region in high quality, the video must be encoded in short segments (\eg every one second, as opposed to every 4-8 seconds in non-\vr videos) and spatially split into many tiles, which introduces a substantial compression overhead and diminishes the bandwidth savings.
%\footnote{Moreover, }
Third, streaming the viewport still consumes more bandwidth than streaming non-\vr videos, as a viewport in the \vrvideo display (98\textdegree-by-100\textdegree) is much larger than the size of a laptop/smartphone screen in the view of a user.
% \xinggong{we don't address this issue yet, changed to: Cropping frames to many fine-grained tiles introduces large compression overhead}
%But other than the above factor, the assumed QoE model remains largely the same, and this fundamentally limits the room for improvement of \vr videos.

This work explores a different dimension than the viewport-driven approach: instead of assuming \vr video users perceive the video quality in the viewport in the same way as watching non-\vr videos, we show that \vr video quality is often perceived {\em differently} than traditional video quality.
% contrary to the conventional belief, 
%the 360\textdegree{} view depends only on its distance to the viewpoint and the encoded quality level, 
Our empirical experiments show that the perceived quality of a \vr video is heavily influenced by several \vrvideo-specific factors, including the {\em speed} of the head movement, the {\em changes of depth-of-field} and {\em luminance} of objects in view due to head movements.
%, compared to those the user have just watched. 
% It is important to notice that these factors are driven by ``user actions'', which are predominant only in \vr videos.
%That is the viewport position and video quality, we found that a \vr video at least three reasons: the speed of {\color{red} head movement}, how the relative depth of the viewed objects, as well as the brightness of the objects compared to those the user have just watched. 
For instance, when shown the same video encoded at different quality levels, the viewer is sensitive to even small quality distortion when the viewpoint is static or moves slowly (\eg $<$5 degree/second); however, the sensitivity drops sharply when the viewpoints move quickly (\eg shaking head or browsing the landscape). 
In short, the sensitivity of users to quality distortion {\em varies} over time by the ``user actions'', which are predominant only in \vr videos.
(See \S\ref{subsec:opportunities} for more discussions.)
%Similarly, how sensitive the viewer is to a quality distortion depends greatly on how further/closer the object is or how much brighter/darker compared to objects that the viewer just saw.



These \vrvideo-specific insights on quality perception open up
%that humans have only bounded sensitivity to quality degradation can 
% have great implications for the design of a more efficient \vr video streaming system. 
new avenues to improveing \vr video quality and bandwidth savings.
% With a deeper understanding of how user perceive the video quality,
If we know exactly how sensitive the user is to the quality distortion at any moment, we can raise quality level always by a maximally perceivable amount, when there is spare bandwidth; and lower the quality level always by a minimally perceivable (or imperceivable) amount, when the bandwidth is insufficient.
Based on an empirical study over 50 \vr videos and 20 actual viewers, we found that one can save 50\% bandwidth without any drop in perceived quality (\S\ref{subsec:potentials}).
% \guanyu{JC: figure of potential improvement has no information about buffering.}
The key to these opportunities is that people have a limited span of attention.
For instance, as a viewer moves the viewpoint, it does increase the area that has to be streamed, but the viewer's attention ``per-pixel'' drops as a result of having to spread the limited span of attention across a wider region in the same duration in time. \footnote{This is in similar spirit to the concept of ``Just Noticeable Difference'' (JND)~\cite{brain,JND} in experimental psychology---the minimal visual difference perceivable by humans.} %\eg viewers generally have larger JND when watching a more complex scene. 
But existing JND models focus on the content-level factors (\eg impact of content complexity~\cite{PSPNR}), as opposed to those driven by \vrvideo user actions. 

\begin{figure}
  \centering
  \includegraphics[width=0.3\textwidth]{figures/BufferRatioGraph-eps-converted-to.pdf}
  \caption{\small Performance of \name and the popular viewport-driven approach on 18 \vrvideos and 804 real-user viewpoint traces over an emulated cellular network link of 1.0($\pm$0.3) Mbps.
  Full results are in \S\ref{sec:eval}. %\jc{move the legend to the bottome-middle. change ``pano'' to ``Pano (this work)''. move ``better'' to the bottom right (now it looks like pointing at the grey line)}
  %\jc{replace this with the new graph!}
  }
  \vspace{-0.5cm}
  \label{first_image}
\end{figure}

%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=2.5in]{images/improvement-eps-converted-to.pdf}
%  \caption{Effectiveness of \name at reducing the bandwidth consumption and improving QoE. \jc{TODO. an example graph with two curves comparing \name and a canonical \vr video streaming protocol. }}
%  \label{fig:intro-improvement}
%  \end{figure}



We present {\em \name}, a \vr video streaming system that explores the aforementioned opportunities.
The design of \name makes three specific contributions.

% \vspace{0.1cm}
{\em First, \name presents a new quality perception model (\S\ref{sec:jnd}) that systematically incorporates the new quality-determining factors specific to \vr videos.}
Based on an IRB-approved user study, we quantify the impact of viewpoint-moving speed, relative depth-of-field, relative luminance on viewer's sensitivity to quality degradation. 
% In addition, we also take distance-to-viewpoint (commonly used in prior work) as a factor that affect the QoE.
% We call the resulting JND model as {\em \vrjnd}. 
The resulting quality perception model can estimate, for any given video and viewpoint trajectory, the user mean opinion score more accurately than traditional video quality index (\eg PSNR~\cite{PSNR}).
%the minimal quality degradation likely be perceivable by the viewer.
% A useful empirical finding is that the impact of these factors on user perceived quality is largely independent to each other, which avoid the need to to explore the space of an exponential number of combinations of multiple factors.
%the modeling of impact of multiple factors on JND, which would otherwise have to explore the space of an exponential number of combinations of multiple factors.
%Their likely independence might explained by \jc{what's the intuition here?}


% \vspace{0.1cm}
{\em Second, \name uses a novel variable-size tiling scheme (\S\ref{sec:tiling}) flexible enough to fully optimize the user perceived quality.}
A \vr video is spatially split into tiles, each encoded in multiple quality levels, so that during video playback, the player can flexibly stream the tiles in different quality levels.
%To best utilize the proposed \vrjnd framework, 
%the video encoding should allow different quality levels be applied to different regions in cognizant to the spatial distribution of \vrjnd values.
We show that existing equal-sized grid tiling (\eg 12$\times$6) is suboptimal---a tile can be too coarse-grained (unable to switch the quality level whenever the user sensitivity varies\guanyu{is it right?}) or too fine-grained (too much encoding/compression overhead).
%In fairness, the square tiling is designed to serve only one purpose of differentiating regions closer to the viewport center from the rest.
Instead, \name splits the \vr video into square tiles of different sizes, which roughly match the spatial boundaries between different levels of user sensitivities.
% Each tile is encoded in multiple levels of quantization parameter, or QP as in prior work.
In some sense, it strike a balance between encoding individual fine-grained objects separately and today's simple grid tiling.



% \vspace{0.1cm}
{\em Finally, \name adapts video quality (\S\ref{sec:control}) in a way that is (a) robust to randomness of viewpoint movements, and (b) readily deployable over the existing video delivery infrastructure.}
At first glance, using estimated user action to drive quality adaptation can be susceptible to prediction errors of head movements. 
Surprisingly, we found the quality adaptation logic can tolerate a fair amount of prediction errors of user actions (\eg viewpoint-moving speed), by leveraging the fact that, to pick the best quality level, it suffices to predict the {\em range} of viewpoint-moving speed, rather than its exact value.
%a region remains almost same for a range of actions (\eg \vrjnd remains the same as long as the viewpoint speed is over a threshold), so what we need is to not to accurately predict the exact trajectory of the viewpoint, but rather the {\em range} of user actions.
\name also addresses a practical challenge that, to accurately estimate the user's real-time sensitivity to quality distortion, \name needs information from the client (the viewpoint trajectory) as well as the server (the pixel-level video content), making it incompatible with the mainstream client-driven video delivery architecture~\cite{DASH}. 
%on the server (\ie cannot be done by the client itself), so it is incompatible with the mainstream DASH protocols which stream videos from stateless HTTP web servers. 
%to determine the perceived quality of a chunk require some computation based on the video data on the server side, so in theory, it is incompatible with the mainstream DASH protocols which stream videos from stateless HTTP web servers.
%This is not a problem in non-\vr videos or existing \vr video protocols, because calculating the perceived quality of a chunk only depends on the available bandwidth and user viewport, both are locally accessible on the client side.
%However, the perceived quality in \vrjnd depends on the video content and user actions (\ie viewport trajectory and its projection), so the client cannot estimate the user-perceived quality without having the video content in the first place. 
%One approach to this conundrum is to let the video client upload the user action information to the server which then makes adaptation decisions, but this goes against DASH's HTTP-based architecture.
%Instead, in this work, we have taken a pragmatic stance to work within the constraints that have spurred the growth of video traffic---streaming videos from web servers over HTTP, like in DASH.
To make \name readily deployable, we {\em decouple} the bitrate adaptation into an offline phase and an online phase.
The offline phase pre-computes the perceived quality for a few carefully picked user actions, and send these estimates as part of the video metafile to the client when a video session begins;
during playback, the client can estimate the user sensitivity by finding the ``nearest neighbor'' in the pre-computed user actions (\S\ref{subsec:compatible}).
%The basic idea is that it is possible to pre-compute the best quality levels for only a few carefully picked possible values of the user action information (viewport trajectory and its projection), and send these estimates as part of the DASH metafile to the client at the beginning of a video session. 
% In the online phase, the client estimates the user action (as described above) and pick the quality level by the ``nearest neighbor'' among the user inputs that have been pre-computed. 
%The intuition behind pre-computing only a few user-action inputs is an empirical observation that in \vrjnd the impact of the user-action input is non-linear; \eg when the viewport movement speed is over some threshold, its impact on \vrjnd and the QP adaptation changes only marginally (probably because the viewer will be very insensitive).


% \vspace{0.1cm}
We implemented a prototype of \name \edited {based on ffmpeg~\cite{ffmpeg} (streaming and codec), and Unity~\cite{unity} (rendering videos on a curved sphere of head-mounted device).}
%\guanyu{on FFmpeg (for streaming \& decoding) and Unity (for curved sphere mapping \& rendering on Head Mounted Device)}.
%\jc{on what platform}
\edited{Using a combination of user studies (20 users, 7 videos) and trace-driven simulation (48 users, 50 videos), we show that \name significantly improves the perceived bandwidth with less bandwidth consumption.
For instance, across a variety of content genres, \name achieves 25-142\% higher mean opinion score than the state-of-the-art viewport-driven streaming solution.
Trace-driven simulation shows that without drop in perceived quality, \name can save up-to 45\% of bandwidth and 15\%-80\% less buffering ratio.}
% on one content provider with 420 VR video sessions, provided by 20 viewers. Video types includes singing \& dancing, nature, science fiction, sports, documentary, gaming and adventure.

% Our experiments show that \name can save 45\% bandwidth compared with state-of-art 360-video streaming solutions, without decrease of perceived quality.
% %\jc{add a line to describe the final user-rating based end-to-end experiments}
% \guanyu{In our user-rating based end-to-end experiment, given the same network condition, \name improves 45\% to 169\% user rating (mean opinion score) compared with state-of-art 360-video streaming solutions.}



==> motivate_long.tex <==
%!TEX root = main.tex

\section{Motivation}
\label{sec:motivate}

\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.9\textwidth]{figures/examples.pdf}
  \vspace{-5mm}
  \caption{\small Illustrative examples of the three \vr video-specific factor, and how they help save bandwidth by selectively reducing the quality of part of the video without affecting the user-perceived quality. The yellow boxes indicate the viewport (dashed ones are previous viewport). 
In each subgraph, the left-hand side and the right-hand side have similar perceived QoE, despite the quality distortions on some objects.}
  \label{fig:examples}
  \end{figure*}

We start with a background on \vrvideo streaming and today's common approach (\S\ref{subsec:background}).
%a full discussion on related work can be found in \S\ref{sec:related}).
Then, we outline the new observations on how user perceive \vr video quality differently, which inspire new opportunities to improve quality and save bandwidth (\S\ref{subsec:opportunities}), empirically analyze their potential gains (\S\ref{subsec:potentials}), and finally, highlight the challenges that must be addressed to unleash the potential benefits (\S\ref{subsec:challenges}).


\subsection{Background of \vr video streaming}
\label{subsec:background}

%\mypara{\vr video streaming}
%\mypara{\vr videos coming to age}
%\vr video streaming is coming to age. 
%According to eMarketer, 
% By the beginning of 2019, 
There are already 36.9 millions VR users in the US (over 10\% of its population), and the number is expected to increase 70 percent in the next two years~\cite{https://channelfactory.com/blog/youtube-trends-vr-ar-advertising/,eMarketer}. 
%Moreover, Head-Mounted Devices (HMD) for VR display are increasingly popular. 
By 2022, there will be over 55 million active VR headsets in the US, which is as many as paying Netflix members in the US in 2018~\cite{https://qz.com/1298512/vr-could-be-as-big-in-the-us-as-netflix-in-five-years-study-shows/}.
Almost all major content providers (YouTube~\cite{Google}, Facebook~\cite{facebook}, Netflix~\cite{Netflix}, Vimeo~\cite{Vimeo}, Hulu~\cite{Hulu}, iQIYI~\cite{iQiyi}, YouKu~\cite{Google}) have launched \vrvideo {\em streaming} services on multiple  platforms~\cite{oculus,samsung,daydreams,etc}, believing that \vr videos are the future of story telling. 
Users watch $1$M hours \vrvideos per day on Facebook~\cite{facebook}.
%\jc{add more concrete statistics on the popularity of VR}
%\xinggong{Youtube 360 channel~\cite{Google} have contributed $8.5$M panoramic programs with $2.8$M subscribers. One favorite video have been viewed by $70$M times. While in Facebook~\cite{facebook}, users have spent about $1$M hours on \vrvideo per day.}

%\mypara{Delivery architecture} 
The proliferation of the \vrvideo content and devices is spurred partly by the highly efficient and scalable delivery architecture. 
\vrvideos can be cheaply delivered to viewers through commercial CDNs, just as other Internet video traffic.
A \vrvideo is first encoded by a \vr encoder (\eg~\cite{??}), which transcodes and chops the video into segments (or chunks); these video segments are then distributed to geo-distributed CDN servers; and finally, a client player (headset or smartphone) streams the video segments sequentially from the nearby CDN server using standard HTTP(S) (or DASH) protocols~\cite{hls,https://www.wowza.com/solutions/streaming-types/virtual-reality-and-360-degree-streaming}.
%\jc{other than the client-side adaptation scheme, is there some fundamental diff or non-trivial steps involved in the preparation/dissemination of \vr content?}
% \xinggong{Unlike tradition videos with multiple bit-rate versions, \vrvideo have to prepare multiple viewport-dependent version to reduce streaming bitrate. Beside, interactive behaviors of head movement put stringent requirements on network delay and video compression.}   
To handle last-mile bandwidth fluctuations, the video segments are encoded in multiple quality levels (\eg quantization parameters), so that during playback, the \vrvideo player can switch between quality levels at the boundary of two consecutive segments, in much the same way of traditional bitrate-adaptive streaming.
%Like non-\vr videos, \vrvideo streaming needs to cope with bandwidth fluctuation by adapting the quality level in order to strike a balance between video quality and bandwidth consumption.
%\mypara{Existing \vr video streaming protocols}

A distinctive feature of \vr video streaming is that the viewer's attention is {\em unevenly} distributed, with more attention centered around the {\em viewport} (the part of the panoramic space that directly faces the user), whereas non-\vr videos are displayed on a fixed desktop or smartphone screen, so the spatial unevenness of attention is less obvious.
Thus, many \vrvideo streaming techniques (\eg~\cite{Gaddam,Graf,POI360,Flare}) explore the {\em spatial} dimension. 
For instance, they spatially partition each video frame into grid {\em tiles} (in 6-by-12 grids), and encode each in multiple quality levels, so that the \vrvideo player can assign higher quality level for tiles that are closer to the viewpoint (the center of a viewport). % {\em distance-to-viewport} ({\em DoV}), with higher quality in area closer to the user's viewpoint and lower quality for rest of the space.
Despite the demonstrated improvement, this viewport-driven approach have two basic limitations:
%These {\em viewport-driven} protocols (\eg~\cite{??,??,??}) that the user-perceived quality of a spatial region is a function of the encoded quality and the region's distance to the viewport center.
% However, the gain of these {\em viewport-driven} protocols (\eg~\cite{Gaddam,Graf,POI360,Flare}) has 
(1) any prediction error of viewpoint movements can cause the re-buffering, which negatively affect user experience; and 
(2) in order to stream high-quality content in the dynamic viewport, the video must be spatially split into tiles (or encoded with many viewport-specific versions), which introduces a substantial compression overhead and thus diminishes the bandwidth savings.
%video segments must be short (typically one second, as opposed to 4-10 seconds in non-\vrvideos) so that the player can adapt the quality level as the viewpoint moves. \jc{add a concrete number for the size inflation due to the short chunk duration}
%\xinggong{Guanyu~ give a number. Junchen~ should we emphasis this issue? do we solve it? }
%\guanyu{Junchen~ We do not solve this issue. Better to remove this.}
% Despite many viewpoint-driven streaming~\cite{ProbDASH,Hosseini,Duanmu2017Prioritized}, these limitations remains.
%\xinggong{DoV-driven or viewport-driven}



%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=0.5\textwidth]{figures/example-speed.pdf}
%  \caption{Illustrative examples of the first \vr video-specific factor. 
%  Viewers tend to be insensitive to quality distortions of the objects moving at a high speed relative to the viewport, which can be (a) an object moving across a static viewport, or (b) the viewport moving across a static background. The yellow boxes indicate the viewport. 
%  In (a) and (b), the left-hand side and the right-hand side have similar perceived QoE, despite the quality distortions on some objects.}
%  \label{fig:example-speed}
%  \end{figure}
%
%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=0.5\textwidth]{figures/example-luminance-fov.pdf}
%  \caption{Illustrative examples of the 2nd and 3rd \vr video-specific factors. 
%  Viewers tend to be insensitive to quality distortions when (a) adapting to changes in luminance and when (b) an object has a different field-of-depth to the viewport.
%  The dashed boxes and solid boxes indicate where the viewport was and where it is now, respectively.
%  In both sub-figures, the left-hand side and the right-hand side have similar perceived QoE, despite the quality distortions on some objects.}
%  \label{fig:example-luminance}
%  \end{figure}

\subsection{New quality-determining factors}
\label{subsec:opportunities}

A key premise behind the prior work is that users perceive the quality of \vr videos (in the viewport) in the same way as they perceive the quality of non-\vr videos, which fundamentally limits their room for improvement by the bandwidth-quality tradeoffs of traditional videos.
Contrary to this assumption, our key insight is that the perceived quality of \vr videos can be heavily influenced by factors (head movements) that are unique to \vr videos, thus opening up new opportunities to improve over existing work.
%The driving intuition behind this work is that 
%prior work has assumed users perceive the quality of the \vr video within in the viewport in much the same way as they perceive the quality of non-\vr videos, where as 
%Through a deeper understanding of how viewers perceive \vrvideo quality, one can improve video quality or save bandwidth consumption without drop in perceived quality.
In particular, we found three {\em \vrvideo-specific quality-determining factors} not yet considered by existing solutions (see \S\ref{sec:jnd} for more analysis on these factors.)
%While the uneven distribution of the viewer's attention affects the QoE-bandwidth tradeoff, our first key observation is that it is just one of {\em several \vr video-specific factors that can heavily influence the perceived QoE of \vr videos but have yet to be fully explored}. 
%In particular, this paper examines the three following factors:

%\jc{need to visualize the three factors}

\begin{packeditemize}

%\myparashort
\item {\bf Factor\#1: Viewpoint-moving speed.} 
%A key feature of \vr videos is that users can freely move their viewpoints. 
As the viewer moves her viewpoint, it also reduces the sensitivity to the quality distortion; and intuitively, the higher the speed, the lower the sensitivity. 
Figure~\ref{fig:examples}(a) gives an illustrative example of how this observation helps save bandwidth: when the viewer moves the viewpoint (\eg to track a moving object, as in the example), we found that reducing the quality level of static objects has little impact on user-perceived quality.
We measure the viewpoint-moving speed in \fillme.
%Similarly, when viewport is static, the viewer will tend to be insensitive to quality distortion of fast moving objects. 
%Consequently, as the viewers watch the video while moving their heads, they sometime report higher perceived quality than other static viewer perceive on the same video at the same objective quality level.
%the perceived quality is significantly improved, since user is unable to detect the distortion. 


%\myparashort
\item {\bf Factor\#2: Change in scene luminance.} 
Our second observation is that as the viewer moves her view around, the viewed region may switch between different levels of luminance; when the content changes from dark to bright (and vise versa), users tend to be less sensitive to quality distortion in a short period of time (typically 5 seconds~\cite{??}).
Figure~\ref{fig:examples}(b) illustrates a simple example of how one can carefully lower the quality level of part of the video without causing any drop in the user-perceived quality.
We measure the luminance in \fillme.
%When user wears a HMD in VR display, environmental brightness perceived by eyes is totally depended on luminance of video content itself.  
%As a result, when watching the same content encoded in the same objective quality, people report different levels of subjective quality depending on whether they have just watched something in different levels of luminance.


%\myparashort
\item {\bf Factor\#3: Changes in depth-of-field (DoF).} 
\vr displays can precisely simulate the DoF by projecting an object to the two eyes with a specific binocular parallax (disparity)~\cite{DoF1}. 
Our third observation is that a viewer can only be sensitive to the quality distortion of one of two objects when they have different DoFs %(\eg one being much closer to the viewer than the other).
 %\jc{citation?
Figure~\ref{fig:examples}(c) illustrates that one can reduce quality level of objects that have a different DoF than where the viewer currently looks at\footnote{This paper assumes the object closest to the viewpoint is the one watched by the viewer. This can be imprecise, but it could be improved by standard tracking mechanism (\eg~\cite{??,??})}.
We measure the DoF in \fillme.
%We found that objects with small DoF (\ie closer to the viewer) have greater parallax, which lowers the viewer's sensitivity to quality distortion due to binocular fusion.
%As a result, a viewer might give different levels of attention to the objects of different DoF's, even if they are all close to the center of the viewport.

\end{packeditemize}
%\jc{why today's videos don't use them.}

%\noindent We want to make two remarks on these opportunities.

\mypara{Intuitive explanation}
The key to these opportunities is that a user has {\em a limited span of attention}.
With the new features of panoramic view and immersive experience, the video size grow dramatically, but the span of attention remains largely constant\footnote{The span of attention does grow as the \vr headset shows a bigger virtual screen, but this is a much smaller increase compared to the size inflation of the whole \vrvideo.}. 
Consequently, a viewer will give less attention to the specifics of a \vr video, which in turn reduces her sensitivity to any quality distortion.

\myparaq{What is new about them}
While these factors %\xinggong{traditional 3D video also has DoF} 
have been studied in the context of other videos, their potential benefits and applications are broadened in \vr videos by the free movements of the headset and viewport. 
For instance, while it is well known that lowering the quality of fast-moving objects has little impact on user experience, \vr videos can benefit from this fact differently than traditional videos: if a \vr video viewer moves her head to track a moving object, the whole background now becomes a ``moving'' object, and thus can tolerate lower quality without affecting user experience.
Note that these factors are not directly captured in viewport-driven techniques which treats objects with the same distance-to-viewport equally.
%For instance, in non-\vr videos, fast-moving parts of the video may be given lower quality than static parts, but \vrvideos open up new opportunities as the viewer may actually look at the moving object, thus one can use lower quality for the whole background. 
%On the other hand, these factors are certainly different to traditional viewpoint-driven streaming adaptation, which assumes the user-perceived quality only depends on the distance-to-viewpoint. 


%creating a multitude of room for improving the bandwidth-QoE tradeoffs, including viewport-driven adaptation as well as the three aforementioned factors.


%\jc{
%\begin{itemize}
%\item p1: we first extend the jnd model with several \vr specific factors, 1, 2, 3
%\item p2: with the new jnd model (explained latter), the potential improvement is tremendous!
%\end{itemize}
%}




%The uneven distribution of \vr user's sensitivities can be explained by the attention theory~\cite{??,??}, which has been successfully applied to specialized video encoder and human-computer interface. 
%The key concept is the just-noticeable difference (JND)---a user tends to notice the difference between two images/videos, only after the difference is greater than a threshold of JND, which depends heavily on the image/video content (as well as the context of the viewer).
%\jc{add a few examples of JND, like content luminance, texture complexity}

%The existing viewport-driven streaming protocols can be seen as one design point of using JND which only depends on the distance between a region and the viewport center. 
%We have seen a few efforts to introduce the existing JND-based attention models in video streaming~\cite{??,??}, although so far their real application so far has been quite limited.


\subsection{Potential for improvement}
\label{subsec:potentials}

We use a real-world dataset to demonstrate the potential gains by leveraging the new quality-determining factors.

\begin{table}[t]
\begin{small}
\begin{tabular}{rcccc}
 \hline
{\bf Types} & Shows & Sports & Nature & Others\\ \hline
{\bf \# of videos} & 5 & 4 & 3 & 6 \\ \hline
{\bf Total duration (mins)} & \fillme & \fillme & \fillme & \fillme \\ \hline
{\bf Full resolution} & \multicolumn{4}{c}{2880 by 1440} \\ \hline
{\bf Frame rate} & \multicolumn{4}{c}{30 FPS} \\ \hline
{\bf \# of views per video} & \multicolumn{4}{c}{48} \\ \hline
%Original resolution & \multicolumn{4}{c}{2880 by 1440} \\ \hline
%Duration & \multicolumn{4}{c}{1$\sim$8 minutes} \\ \hline
%Frame rate & \multicolumn{4}{c}{30 FPS} \\ \hline
%Views per video & \multicolumn{4}{c}{48} \\ \hline
\end{tabular}
\end{small}
\caption{\small Dataset summary 
%\jc{break it down by genres, add the user info}
}
\label{tab:dataset}
\end{table}


\mypara{Dataset}
The dataset consists of 18 \vrvideos, each watched by 48 users using\fillme device~\cite{??}.
The video dataset 
%was provided by \cite{VRdataset}, and it 
can be found in ~\cite{VRdataset_page}. %\jc{is there a public source?}
%Each video was played by a virutual reality head-mounted device~\cite{??}
The video content covers three major categories: shows (5), sports (4), nature (3).
Table~\ref{tab:dataset} gives a summary of the dataset.

\myparaq{How prevalent are these factors}
We first measure the prevalence of the impact of the three new quality-determining factors. 
Figure~\ref{fig:prevalence} shows the distribution of viewpoint-moving speed, luminance changes in a small time window, and DoF differences among objects in the viewport. %(which will not be differentiated by existing techniques).
As we will see in \S\ref{subsec:jnd:details}, the impact of each of these factors on perceived quality has a ``threshold'' effect: the viewer's sensitivity to quality distortion will drop significantly, if the viewpoint-moving speed is over 20 degree/s, luminance of viewpoint object changes by over 80 gray level, or the object's DoF differs to the viewpoint object by over 0.3 \jc{in what unit?}.
We can see that all of these factors exceed their thresholds (\ie lowered user sensitivity to quality distortion) for a substantial fraction of time.
For instance, for more than 25\% of the time, the viewpoint moves faster than 20~degree/s, which means the viewers are unlikely to perceive a 80\% drop in quality of the static background content (see \S\ref{subsec:jnd:details}).
%Similarly, %\jc{a sentence on the other two graphs.}
%\xinggong{the occurrence ratio of luminance changes larger than 80 gray level is about 50\%, and that of DoF difference(>0.3) is about 55\%.} 


%%According to our data analysis, more than \fillme\% time, user's viewpoint is moving faster than \fillme \textdegree/s. 
%One of the most highlighted feature of VR video is that users can freely move their viewpoints. According to our data analysis, more than 30\% viewpoints are moving faster than 20 deg/s. (Fig. \ref{CDFspeed}) 
%When human viewpoint is moving, visual acuity is decreased in 2 different conditions: (1) if user is tracking an object, visual acuity decreases smoothly with viewpoint moving speed increases. (2) If user is not tracking an object, visual acuity decreases dramatically with viewpoint moving speed increases. \cite{speed}
%\jc{can you visualize such findings, and also show some numbers about the other two factors?}

\begin{figure}
  \centering
  %\includegraphics[width=0.5\textwidth]{figures/prevalence.pdf}
   \begin{minipage}[t]{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/Figure3a-eps-converted-to.pdf}
%{(a) Client-side CPU overhead}
\label{fig:side:a}
\end{minipage}
\begin{minipage}[t]{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/Figure3c-eps-converted-to.pdf}
%{(b) Video start-up delay}
\label{fig:side:b}
\end{minipage}
\begin{minipage}[t]{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/Figure3b-eps-converted-to.pdf}
%{(c) Pre-processing time for a 1 minute video}
\label{fig:side:c}
\end{minipage}
  \caption{\small Prevalence of the new opportunities. \jc{bigger font}}
  \label{fig:prevalence}
 \end{figure}


\newcommand{\ideal}{Ideal\vr \xspace}

\mypara{Potential gains over viewport-driven approach}
Since that users are insensitive to video quality for a substantial fraction of time, it is natural to strike a better quality-bandwidth tradeoff by spending more bandwidth on when/where users {\em are} sensitive to the quality distortion.
To demonstrate this potential gain, we consider a canonical viewport-driven baseline as the reference, and a new \vr video streaming scheme, called {\em \ideal}.
In both schemes, we split each frame into 6$\times$12 grid tiles, encode each tile in \fillme quality levels (QP=\{\fillme,\fillme,\dots\}) values, and give low quality to tiles outside of the viewport. 
The difference is that when deciding the quality level of each tile {\em within} the viewport, the baseline gives the highest possible quality level (below the available bandwidth constraint), but \ideal uses the lowest quality level, if any of the new factors exceeds its threshold in Figure~\ref{fig:prevalence} (\ie viewpoint-moving speed over 20 degree/sec, change of luminance of viewpoint object over 80 gray level, or the difference between its DoF to the viewpoint DoF over 0.3 D).
For a fair comparison, we assume the viewpoint position and available bandwidth are known in both schemes.


\begin{figure}
  \centering
  \includegraphics[width=2.5in]{figures/Figure4-eps-converted-to.pdf}
  \caption{PSPNR-bandwidth tradeoff of (1) Viewpoint-driven VR streaming. (2) Perceived quality driven VR streaming. (3) Perceived quality driven VR streaming. (with 3 VR factors)\jc{NEED TO BE UPDATED}}
  \label{fig:potential}
  \end{figure}

Figure~\ref{fig:potential} compares the bandwidth consumption and user-perceived quality (measured in a custom PSPNR index, which as we will show in \S\ref{sec:jnd} has a stronger correlation with subjective user rating than alternative measures). 
We vary the available bandwidth to plot a wide range of quality-bandwidth tradeoffs.
The figure confirms our intuition that \ideal reduces bandwidth consumption with little impact on user experience. 
%this intuition that the idealized \vrvideo achieves a much better quality-bandwidth tradeoffs than the DoV-driven baseline.
%We use peak signal-to-perceptible-noise ratio (PSPNR)~\cite{PSPNR} as an indicator of the perceived quality. 
%We will discuss PSPNR in full details in \S\ref{sec:jnd}, but in short, it has a stronger linear correlation to subjective user rating than alternative measures (\eg PSNR).
The idealized \vrvideo can save 60\% bandwidth without drop in perceived quality, or improve the perceived quality by 100\% (roughly an 100\% increase in user rating) using the same amount of bandwidth.
It should be noticed that both schemes are idealized (viewpoint trajectory and bandwidth are known in advance), but their comparison is indicative of the potential improvement of using the three new factors. 


%\guanyu{A video is cut to 6 $\times$ 12 tiles, with each tile 5 quality levels. We check all tiles in viewport, for each of the 3 new factors illustrated in Figure~ \ref{fig:prevalence}, when user's actual behavior exceeds the red line, we lower 1 quality level of this tile. We do the same thing on factors considered in traditional video (luminance, distance from content to viewpoint, texture complexity).}
%%\jc{need details, how many quality levels? how many tiles? how to allocate quality levels under a given bandwidth?}
%%\xinggong{It is able to tile frame and allocate bitrate by the new quality-determining factors.}   
%We compare it with a baseline inspired by the common DoV-driven approach: each frame is split into 
%6*12 equal-sized rectangular tiles\footnote{\jc{how do we handle the problem of curved sphere? did we use any standard techniques?}}, and the tile covering the viewport are given the highest quality level, %\jc{and how to allocate the rest tiles?}
%\guanyu{for the tiles out of viewport, we leave it empty. For all above methods, user's viewport can be always predicted correctly. }



%Before giving the concrete design of an actual streaming protocol, we first present the potential for improvement of leveraging the \vr-specific factors. 
%To do so, we use a metric called PSPNR to denote the perceived quality of a viewer, which can be expressed by $F(P,P',A,v,d,\Delta d,l,\Delta l)$, where $P$ and $P'$ denote the original frame and the rendered frame respectively, $a=(x_a,y_a)$ the viewport center, $v$ the viewport moving speed, $d$ the DoF, $\Delta d$ the change in DoF, $l$ the luminance, and $\Delta l$ the change in luminance. 
%We will explain this metric in greater detail in the next section. 
%\jc{give a short description of how to understand PSPNR}

%PSPNR \cite{PSPNR} is applied as a metric to measure perceived quality. Real traces are collected from over 800 VR displays of 48 users. In our experiment, each video has 5 different bitrate level. We compare the performance of 3 methods:
%\begin{itemize}
%
%\item \emph{Viewpoint-driven VR streaming.} Video is cut into 6*12 spatial rectangular tiles. Tiles on user's viewpoint is allocated the high bitrate. For other tiles, bitrate is allocated linearly decreasing with its distance to user's viewpoint.
%
%\item \emph{Perceived quality driven VR streaming. (with 3 VR factors)} Suppose we can freely allocate bitrate to each spatial part of video without video tiling. Besides user viewpoint, content luminance and texture complexity, we also take consideration of viewpoint moving speed, content Depth-of-Field and light / dark adaptation, we do adaptive streaming to maximize user-perceived quality.
%
%\end{itemize}
%
%With consideration of content luminance and texture complexity, perceived-quality-driven VR streaming can save 30\% bandwidth compared with viewpoint-driven VR streaming providing the same PSPNR. Moreover, when we take consideration of viewpoint moving speed, object Depth-of-Field and light / dark adaptation, we can further save 20\% bandwidth.






\subsection{Key challenges}
\label{subsec:challenges}

However, to fully explore these opportunities requires not only changing the quality objective function, but re-architecting several critical components of the video delivery pipeline. 
In particular, we identify three main challenges.

%In order to achieve perceived quality driven VR streaming, the core challenge is: perceived quality is related to both video content and user behavior, how to take together both-sides information to maximize the perceived quality. For specifically, there are three aspects:

\myparashort{Challenge 1: How to leverage the new quality-determining factors in \vrvideo streaming?}
%Challenge 1: Traditional Human Visual System (HVS) models can not measure perceived quality in VR video display.
Before designing the streaming protocol, we first need to incorporate the new quality-determining factors to how \vrvideo quality is measured. 
This, however, is not trivial, as most traditional video quality metrics focus on the impact of content-level dynamism (\eg users are relatively insensitive to quality distortion on a ``busy'' scene) while assuming the viewers are static.
On the contrary, the new quality-determining factors are driven mostly by user actions. 
So our first step is to incorporate them in existing video quality metrics.
%Perceived quality can be well-measured in traditional video display by building mathematical model from luminance, texture complexity and viewpoint-object distance to perceived quality. However, as we have mentioned, besides these existing factors, perceived quality in VR display is related to several new factors which are never modeled before. Their mathematical relationship to perceived quality, and how these new factors combined with existing factors together influence perceived quality are unknown problems.

\myparashort{Challenge 2: How should the \vrvideos be spatially tiled to fully exploit the new opportunities?}
%Challenge 2: Traditional grid-like video tiling scheme performs poorly in perceived quality optimization.
Second, the spatial tiling of \vrvideos must allow enough flexibility so that the quality adaptation logic can differentiate spatial regions to which the viewer has different sensitivity. 
For instance, it is ideal if the tiling is such that objects moving at different speed (\eg foreground vs background) can be assigned with different quality levels.
At a first glance, this can be done by using more fine-grained tiling, but this is not practical as finer-grained tiling will inevitably reduce video  coding efficiency and thus drastically inflate the bandwidth consumption.
Figure~\ref{fig:bitrate-efficiency} shows the average size inflation of all videos in the dataset (the tiled video size over the original video size), and that the size grows almost linearly with the number of tiles. 
So the existing equal-sized tiling mechanism is not sufficient to fully explore the new opportunities.

%To optimize perceived quality, we need to independently allocate bitrate of each spatial part of the video. Grid-like tiling scheme is a widely used method to solve the problem. Video is cut into several rectangular tiles with equal size which can be independently encoded / decoded. So we can allocate different bitrate to different tiles.
%
%However, traditional grid-like tiling performs poorly in perceived quality optimization in two aspects: 
%
%(1) Coarse-grained tiling causes coarse-grained rate allocation, and perceived quality obtained by coarse-grained rate allocation is far from that obtained by fine-grained rate allocation. We encode the video with different rate allocation granularity. We apply PSPNR to measure perceived quality and Fig. \ref{optimalencoding} shows the PSPNR-bandwidth tradeoff. Rate allocation with 3*6 / 6*12 granularity obtains -x\% / -x\% PSPNR compared with 12*24 granularity, this is a significant performance gap in perceived quality optimization.
%
%\begin{figure}
%  \centering
%  \includegraphics[width=2.5in]{images/optimalencoding-eps-converted-to.pdf}
%  \caption{PSPNR-bandwidth tradeoff in video encoding with different granularity of rate allocation.}
%  \label{optimalencoding}
%  \end{figure}
%
%(2) Fine-grained tiling introduces serious bitrate efficiency problem in video encoding. In practice, each tile has to be encoded independently instead of encoded together. When we cut the video into tiles, the total video size is increased. Fig. \ref{bitrateefficiency} shows the video size of different tiling granularity compared with original video size. We find that cutting a video into 12*24 tiles introduces 50\% to 330\% additional video size compared to original video. This significantly lower its practical performance in perceived quality optimization, especially in low bandwidth situations where the bitrate efficiency problem is very serious.

\begin{figure}
  \centering
  \includegraphics[width=0.22\textwidth]{figures/Figure5-eps-converted-to.pdf}
  \caption{The average video size under different tiling granularities.
  \xinggong{curves for the three genres and one average}
  %\jc{pick one line. no need for five lines}
  }
  \label{fig:bitrate-efficiency}
  \end{figure}

\myparashort{Challenge 3: How to design a streaming protocol that is robust to noises in user action and compatible with the existing delivery infrastructure?}
%Challenge 3: Information needed for perceived quality computation is disparted on server-side and client-side.
Finally, the new quality-determining factors call for a revisit on the streaming protocol. 
On one hand, it seems the protocol must be sufficiently adaptive to cope not just fluctuation in bandwidth variation and viewpoint movement, but also real-time changes of the movement speed, the scene luminance, and the depth-of-field. 
On the other hand, the streaming protocol must also be architecturally compatible with the HTTP-based delivery infrastructure that has spurred the rise of \vrvideos, so the quality adaptation is driven solely by the client (while the server passively server the video as web objects). 
Unfortunately, this is difficult because, as we will see, to calculate the optimal quality level, the client needs the knowledge of the video content before streaming the content (unlike in viewpoint-driven scheme). 

%To optimize perceived quality, client needs to compute the perceived quality of each bitrate allocation and then make decision. However, different from video quality which only related to video content itself, perceived quality depends on both video content and user behavior. Information of video content is located on server-side while information of user behavior is located on client-side. To get information of video content with current DASH, client has to pre-request in information of each pixel from server. This communication overload even exceed the overload of actual video streaming.




